Controlling the Depth, Size, and Number of Subtrees for Two-variable Logic on Trees

Verification of properties of first order logic with two variables FO2 has been investigated in a number of contexts. Over arbitrary structures it is known to be decidable with NEXPTIME complexity, with finitely satisfiable formulas having exponential-sized models. Over word structures, where FO2 is known to have the same expressiveness as unary temporal logic, the same properties hold. Over finite labelled ordered trees FO2 is also of interest: it is known to have the same expressiveness as navigational XPath, a common query language for XML documents. Prior work on XPath and FO2 gives a 2EXPTIME bound for satisfiability of FO2. In this work we give the first in-depth look at the complexity of FO2 on trees, and on the size and depth of models. We show that the doubly-exponential bound is not tight, and neither do the NEXPTIME-completeness results from the word case carry over: the exact complexity varies depending on the vocabulary used, the presence or absence of a schema, and the encoding used for labels. Our results depend on an analysis of subformula types in models of FO2 formulas, including techniques for controlling the number of distinct subtrees, the depth, and the size of a witness to finite satisfiability for FO2 sentences over trees.

==> app-oldlowerproof.tex <==

\section{old Proof of Theorem \protect{\ref{fulllower}}}

We will
reduce from the acceptance
problem for  an alternating EXPTIME machine.
We assume, w.l.o.g, that each non-deterministic choice consists of two possible transitions. 
Given a machine we construct a formula $\varphi$ of polynomial size s.t 
$\varphi$ is satisfiable iff $M$ accepts $w$.
Let $M_w$ denote the machine $M$ hardcoded to include $w$ as an input.

To get an idea of the intended encoding we first describe the encoding of a configuration:
A configuration is a `snapshot' of the tape at a particular point. 
Note that we can assume, w.l.o.g, that the maximum space used in the tape is 
bounded by $2^n$, where $n$ is the size
of the input
% as the time bound is $2^n$ and it is known that $ATIME(f(n)) \subseteq DSPACE(f(n))$. 
We therefore describe a  configuration
by an exponential path of nodes. 
 Each node describes a tape position, and the symbol present at that position.
Further we have a special atomic proposition $H$, s.t $H$ is true at only one tape position, and asserts that the head is 
at that position of the tape. To fully describe a configuration we also have to describe the state at which we are 
at. We do so by adding an atomic proposition, $q_i$ (assuming we are state state $q_i$), for all nodes in the configuration. 

The Turing machine computation can now be described as a tree
of configurations starting from the initial configuration.
The tree described by the formula will be a coding of the computation
tree,  with nodes that representing the control state and
configurations represented  by linear segments going from one control
state node to another.
If the state of the configuration is an $\wedge$-state, the
corresponding node in the tree will be forced
to have  two children, each rooting linear sequences
representing  configurations.
For an $\vee$-state, the corresponding node
will have  a single child, rooting
a representation of one of the allowed  configurations. 
 %The children then describe a configuration as described above. 

If the state is an \emph{accepting} state, then we also label the nodes in that configuration with an atomic proposition $A$ (for accepting), and if
it is rejecting we label them with an atomic proposition $R$ (for rejecting). 

To check if $M_{w}$ accepts empty input it is now enough to check that none of the configurations are ever rejecting, simply asserting that none of the nodes are ever labelled $R$. If such a model exists then we have that the initial configuration is accepting (according to the rules above). This is because no matter what path we follow
we will reach an accepting configuration. This construction is illustrated in Figure \ref{fig:apspace}.
\input{DIAG4}

We now describe the construction formally:
Note that the number of configurations chosen is exponential in the size of the input $n$; Say this is, w.l.o.g, $E = 2^n$. 
We describe the configuration of a node $x$ using binary representation. We use atomic propositions $c_1, \dots, c_n$ to describe a configuration number
from $0$ to $2^n-1$ (When $c_i$ is true at a node its bit is 1 and when false it is 0). Note that
this binary representation doesn't encode all configurations in the tree
but rather the configuration visited in any run. At each nondeterministic choice we have a different child for each of the two possible next configurations, but have the same binary representation for both.
In a similar fashion, we use atomic propositions $p_1, \dots, p_n$ to describe the tape position of node $x$ within a configuration. 
Let $T_{\alpha}$ be the atomic proposition saying that node $x$ has symbol $\alpha$. Similarly let $H$ be the atomic proposition for saying the head is at tape position
$x$. 
This describes the set of atomic proposition used. 
% More atomic propositions used

We now describe a number of encodings. 
Two nodes are within the same configuration (tape positions of same configuration):
\[ \text{SameConf}(x, y) = \bigwedge_i (c_i(x) \iff c_i(y) \wedge (x = y \vee x ~ \descof ~  y \vee y ~ \descof ~  x) \] 
We note that subsequent positions or configurations occur only on the same path, so as long as $x$ and $y$ above lie on the same path, 
they must be of the same configuration.

Similarly two nodes have the same tape position (not necessarily in the same configuration) if:
\[ \text{SamePos}(x, y) = \bigwedge_i (p_i(x) \iff p_i(y) ) \] 


The following represents the fact that $x$ and $y$ are positions in the tape just next to each other, within the same configuration:
\begin{align*} 
\text{NextPosInConf}(x, y) & = \text{SameConf}(x, y) \wedge 
              \bigvee_{1 \leq i \leq n} ( 
              \bigwedge_{r < i} (p_r(x) \iff p_r(y)) \\ 
              & \wedge (\neg p_i(x) \wedge p_i(y)) 
               \wedge \bigwedge_{r > i}  (p_r(x) \wedge \neg p_r(y))
               )
\end{align*}
In the above we have the binary representation of position $y$ ($p_1\dots, p_n$) is 1 greater than that of $x$ (we look for the position
of the first 0 in the binary representation and then make sure it is set to 1, while the rest behaves appropriately). 

Note that in a special case, where the binary representation is all 1's, this is the last position of the configuration:
\[ \text{LastPos}(x) = \bigwedge_i p_i\]
Similarly the first position is given by:
\[ \text{FirstPos}(x) = \bigwedge_i \neg p_i\]

We now give a formula describing when $x$ and $y$ are in two subsequent configurations:
\begin{align*} 
NextConf(x, y) & = (y ~ \descof  x) \wedge \bigvee_{1 \leq i \leq n} ( 
               \bigwedge_{r < i} (c_r(x) \iff c_r(y)) \\ 
              & \wedge (\neg c_i(x) \wedge c_i(y)) 
               \wedge \bigwedge_{r > i}  (c_r(x) \wedge \neg c_r(y))
              )
\end{align*} 
To ensure that the configuration is indeed a subsequent one, we ensure not
only the bit encoding is 1 greater, but also that y is a descendant of x, ensuring that it is on the same path. 
Otherwise, we could have a node with the same bit encoding on a different path (due to the alternation). This is illustrated in 
Figure \ref{fig:conf}.
\input{DIAG5}
We have that if two nodes $x$ and $y$ are the last and first nodes in a configuration (respectively), and the configuration
of $y$ is 1 greater then that of $x$, then this can be represented as follows:
\begin{align*} 
\text{NextConfNodes}(x, y) & = \text{LastPos}(x) \wedge \text{FirstPos}(y) \wedge \text{NextConf}(x, y)
\end{align*}


Now $\text{Unique}_{\alpha}(x)$ says that $\alpha$ is the unique symbol (from alphabet) at $x$:
\[ \text{Unique}_{\alpha}(x) = T_{\alpha}(x) \wedge \neg \bigvee_{\beta \neq \alpha} T_{\beta}(x) \]

We now describe a number of formulae to be satisfied:

We now wish to say that two nodes next two each other on the tape (NextPosOnConf) are related by each other by a child. 
Further we say that two nodes related by NextConf are related by a child relation. 
Further it is enough that only these nodes are related by a child relation, so we have:
\[ \varphi_1 = \forall x, y (\text{NextPosOnConf}(x, y) \vee \text{NextConfNodes}(x, y) \iff x ~ \childof ~  y ) \]

We say that all nodes have a unique symbol labelling:
\[ \varphi_2 = \forall x (\bigvee_{\alpha} \text{Unique}_{\alpha}(x) )  \]

Further we require that for each configuration there is a unique node satisfying $H$ (i.e head is at a unique position
in the tape):
\[ \varphi_3 = \forall x \exists y ( (\text{SameConf}(x, y) \wedge H (y) )
                        \wedge \forall x ((\text{SameConf}(x, y) \wedge x \neq y)  \Longrightarrow \neg H(x))) \]
%USING NOT HERE - CHECK THIS OR CHANGE LATER

We now say that each node in a configuration has a unique state $q_i$ and all nodes in the configuration have that state:
\[ \varphi_4 = \bigvee_i \forall x, y ( \text{SameConf}(x, y) \Longrightarrow \text{UniqueState}(x, y, i) ) \]
where:
\[ \text{UniqueState}(x, y, i) =  q_i(x) \wedge q_i(y) \bigwedge_{j \neq i} \neg (q_j(x) \vee q_j(y))  \]

Let $q_a$ be a state labelled with \emph{accept} and $q_r$ a state labelled with \emph{reject}. Then:
\[ \varphi_5 = \bigwedge_a \forall x ( q_a(x) \iff A(x) \]
\[ \varphi_6 = \bigwedge_r \forall x ( q_r(x) \iff R(x) \]
So we have that all nodes of accepting configurations are labelled A, and similarly for rejecting configurations. 

We now enforce that we move from one configuration to the next one(s) correctly:

First we ensure that all positions on the tape apart from the one currently pointed by the head are unaffected:
\[ \varphi_7 = \forall x, y (\text{SamePosInNextConf}(x,y) \wedge \neg H(x) \Longrightarrow \bigwedge_ {\alpha} (T_{\alpha}(x) \iff T_{\alpha}(y))) \]
where SamePosInNextConf represents that $x$, $y$ are in two the same tape positions in subsequent configurations:
\[ \text{SamePosInNextConf}(x,y) = \text{NextConf}(x, y) \wedge \text{SamePos}(x, y) \]

We now ensure configurations change in accordance to the transition function. Assume $q_i$ below with a $\wedge$ or  $\vee$ labelling 
(i.e take only $i$ s.t $v(q_i) = \wedge$ or $v(q_i) = \vee$):
\begin{align*}
\varphi_8 = \forall x, y (\text{SamePosInNextConf}(x,y) \wedge H(x) \Longrightarrow \\
\bigwedge_{i, \alpha} (T_{\alpha}(x) \wedge q_i(x) \Longrightarrow 
     \bigvee_{j=1,2} (F_{\delta_j(q_i, \alpha)}(y) \wedge \forall x (\text{SameConf}(x, y) \wedge A_j(x)))
\end{align*}

where $\delta_j(q_i, \alpha) = (\beta, q_j, X)$ (where $\beta$ is a letter in the alphabet, $q_j$ is some state, and $X$ is either $L$ or $R$)
We have that:
\begin{align*} 
F_{\beta, q_j, L}(y) &=  \exists x (x ~ \childof ~  y \wedge  H(x)) \wedge \forall x (\text{SameConf}(x, y) \wedge q_j(x)) \\
F_{\beta, q_j, R}(y) &=  \exists x (y ~ \childof ~  x \wedge  H(x)) \wedge \forall x (\text{SameConf}(x, y) \wedge q_j(x)) 
\end{align*}
$A_j$ ($j=1, 2$) is a special symbol attached to each of the two subsequent configuration (for all the nodes in the configuration) to identify a 
configuration. This is used below.

Note that the above restricts the subsequent configuration to ones agreeing with $\delta$. Let $q_r$ be states with $\wedge$ labelling and $q_k$ be states with
$\vee$ labelling. We add the following formulas that ensure both configurations occur as children for $q_r$'s and only one subsequent configuration occurs for $q_k$'s:
\[ \varphi_9 = \bigwedge_r (q_r(x) \wedge \text{LastPos}(x) \Longrightarrow
     \exists y (y ~ \childof  ~ x \wedge A_1 (x))
     \wedge \exists y (y  ~ \childof ~  x \wedge A_2(x)) ) 
\]

Similarly we have:
\begin{align*}
\varphi_{10} = &\bigwedge_k (q_k(x) \wedge \text{LastPos}(x) \Longrightarrow \\
      &     ( \exists y (y ~ \childof ~ x \wedge A_1 (x)) \wedge \neg \exists y (y ~ \childof ~  x \wedge A_2 (x))) \\
       &   \vee ( \exists y (y ~ \childof ~  x \wedge A_1 (x)) \wedge \neg \exists y (y ~ \childof ~ x \wedge A_2 (x))) \\
\end{align*}
% MAY CHANGE THIS AS POSITION RIGHT NEXT 11111 JUST BEFORE ALTERNATION MY GIVE A2 CHILD
The only task remaining is to assertion that the initial configuration is true, and enforce that no configuration is rejecting.
For the initial configuration, assume $w = w_0, \dots, w_m$:
\begin{align*} 
\varphi_{11} &= \forall x (C_0 (x) \Longrightarrow q_0(x) \\
       &\wedge ( P_0(x) \Longrightarrow H(x) \wedge (T_{w(0)}(x)) \\
      &\wedge P_1(x) \Longrightarrow (T_{w(1)}(x)) \\
     & \wedge \dots \wedge 
      P_m(x) \Longrightarrow (T_{w_m}(x)) ) )
\end{align*}
where $P_i$ represents position $i$ in the tape (this can be easily converted to binary and converted to a boolean combination in terms of $p_i$'s)
For the second part:
\[ \varphi_{12} = \forall x ( \neg R(x)) \]

Consider the formula:
\[ \varphi = \bigwedge_{i \leq 12} \varphi_i \]
By the above encoding of the alternating Turing machine we have that $\varphi$ is satisfiability iff $M_{w}$ accepts the empty input.

\myparagraph{Modification for $\fotwo[\vdesc]$}
First note that in the prior proof we had included the subformula:
\[ \varphi_1 = \forall x, y (NextPosOnConf(x, y) \vee NextConfNodes(x, y) \iff x ~ \childof ~ y ) \]
% Maybe y < ch x, double check this and below as well
And so we can replace every occurrence
of $x ~ \childof ~  y$ anywhere else in the proof with $(NextPosOnConf(x, y) \vee NextConfNodes(x, y))$.

We now replace  $\varphi_1$ with a different construct. The purpose of $\varphi_1$ is to ensure that configurations
occur in the right order in a path, and that positions within a configuration
occur in the right order. First
we have
\[ \varphi_1 = \forall x, y (NextPosOnConf(x, y) \vee NextConfNodes(x, y) \Longrightarrow x ~\descof ~ y ) \]

Now we also have to ensure that if $x$ is a descendant of $y$, then the configuration of $x$ is lower then that of $y$
or they have the same configuration but the position of $x$ is lower then that of $y$.

\[ \varphi_1' =  (x ~ \descof ~  y) \Longrightarrow BiggerPosInConf (x, y) \vee BiggerConf(x, y) \]
where:
\begin{align*}
\text{BiggerPosInConf} (x, y) &= \text{SameConf}(x, y) \wedge \text{BiggerPos}(x, y)  \\
\text{BiggerPos}(x, y) &= \bigvee_i ((p_i (x) \wedge \neg p_i(y)) \wedge \bigwedge_ {i < j \leq n} p_j(x) \iff p_j(y)) \\
\text{BiggerConf}(x, y) &= \bigvee_i ((c_i (x) \wedge \neg c_i(y)) \wedge \bigwedge_ {i < j \leq n} c_j(x) \iff c_j(y) )
\end{align*}
% Check up to n or up to 0



GIVE MODIFICATIONS FOR RANKED CASE, UNARY ALPHABET CASE

==> generic.tex <==
% packages
\usepackage[english]{babel}
%\usepackage{amsmath,amssymb,amsfonts,mathrsfs,latexsym,stmaryrd}
\usepackage{array}
\usepackage{url}
\usepackage{comment}
\usepackage[newitem,newenum,flushleft,neverdecrease]{paralist}
\usepackage{epsfig}
\usepackage{ifpdf}

% fix for metapost
\ifpdf
  \DeclareGraphicsRule{*}{mps}{*}{}
\else
  \DeclareGraphicsRule{*}{eps}{*}{}
\fi

% environments
\def\labelitemi{\textbullet}
\setlength{\pltopsep}{\smallskipamount}
\setlength{\plitemsep}{\smallskipamount}
\newenvironment{dotlist}{\begin{compactitem}}{\end{compactitem}}
\newenvironment{numlist}{\begin{compactenum}}{\end{compactenum}}
\newenvironment{romlist}{\begin{compactenum}[i)]}{\end{compactenum}}
\newenvironment{condlist}{\begin{compactenum}[{(C}1{)}]}{\end{compactenum}}
\newenvironment{proplist}{\begin{compactenum}[{(P}1{)}]}{\end{compactenum}}
\newenvironment{axiomlist}{\begin{compactenum}[{(A}1{)}]}{\end{compactenum}}
\newcommand{\refeq}[1]{\hyperref[#1]{(\ref*{#1})}}
\newcommand{\refcond}[1]{\hyperref[#1]{C\ref*{#1}}}
\newcommand{\refprop}[1]{\hyperref[#1]{P\ref*{#1}}}
\newcommand{\refaxiom}[1]{\hyperref[#1]{A\ref*{#1}}}
\newcommand{\margincomment}[1]{\marginpar{\small\textit{#1}}}

\providecommand{\qed}{\hfill $\Box$}
\renewcommand{\qed}{\hfill $\Box$}
\newcommand{\eproof}{\qed}

% domains
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbNp}{\mathbb{N}_{>0}}
\newcommand{\bbNinf}{\mathbb{N}\cup\{\infty\}}
\newcommand{\bbNpinf}{\mathbb{N}_{>0}\cup\{\infty\}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbQp}{\mathbb{Q}_{>0}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbRp}{\mathbb{R}_{>0}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbS}{\mathbb{S}}

% classes

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cW}{\mathcal{W}}

% languages
\newcommand{\sA}{\mathscr{A}}
\newcommand{\sB}{\mathscr{B}}
\newcommand{\sC}{\mathscr{C}}
\newcommand{\sD}{\mathscr{D}}
\newcommand{\sE}{\mathscr{E}}
\newcommand{\sF}{\mathscr{F}}
\newcommand{\sG}{\mathscr{G}}
\newcommand{\sH}{\mathscr{H}}
\newcommand{\sI}{\mathscr{I}}
\newcommand{\sJ}{\mathscr{J}}
\newcommand{\sK}{\mathscr{K}}
\newcommand{\sL}{\mathscr{L}}
\newcommand{\sM}{\mathscr{M}}
\newcommand{\sN}{\mathscr{N}}
\newcommand{\sO}{\mathscr{O}}
\newcommand{\sP}{\mathscr{P}}
\newcommand{\sQ}{\mathscr{Q}}
\newcommand{\sR}{\mathscr{R}}
\newcommand{\sS}{\mathscr{S}}
\newcommand{\sT}{\mathscr{T}}
\newcommand{\sU}{\mathscr{U}}
\newcommand{\sV}{\mathscr{V}}
\newcommand{\sX}{\mathscr{X}}
\newcommand{\sY}{\mathscr{Y}}
\newcommand{\sZ}{\mathscr{Z}}
\newcommand{\sW}{\mathscr{W}}

% structures
\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\fZ}{\mathfrak{Z}}
\newcommand{\fW}{\mathfrak{W}}

% objects
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bW}{\mathbf{W}}

% other objects
\newcommand{\tA}{\mathtt{A}}
\newcommand{\tB}{\mathtt{B}}
\newcommand{\tC}{\mathtt{C}}
\newcommand{\tD}{\mathtt{D}}
\newcommand{\tE}{\mathtt{E}}
\newcommand{\tF}{\mathtt{F}}
\newcommand{\tG}{\mathtt{G}}
\newcommand{\tH}{\mathtt{H}}
\newcommand{\tI}{\mathtt{I}}
\newcommand{\tJ}{\mathtt{J}}
\newcommand{\tK}{\mathtt{K}}
\newcommand{\tL}{\mathtt{L}}
\newcommand{\tM}{\mathtt{M}}
\newcommand{\tN}{\mathtt{N}}
\newcommand{\tO}{\mathtt{O}}
\newcommand{\tP}{\mathtt{P}}
\newcommand{\tQ}{\mathtt{Q}}
\newcommand{\tR}{\mathtt{R}}
\newcommand{\tS}{\mathtt{S}}
\newcommand{\tT}{\mathtt{T}}
\newcommand{\tU}{\mathtt{U}}
\newcommand{\tV}{\mathtt{V}}
\newcommand{\tX}{\mathtt{X}}
\newcommand{\tY}{\mathtt{Y}}
\newcommand{\tZ}{\mathtt{Z}}
\newcommand{\tW}{\mathtt{W}}

% shorthands
\newcommand{\s}[1]{\vspace{#1mm}}
\newcommand{\proofskip}{\smallskip\noindent}

\providecommand{\mit}{\mathit}
\renewcommand{\mit}{\mathit}
\newcommand{\mt}{\operatorname}
\newcommand{\mtt}{\mathtt}
\newcommand{\msl}{\mathsl}
\newcommand{\mbf}{\mathbf}
\newcommand{\und}{\underline}

% other objects
\newcommand{\emptystr}{\varepsilon}
\newcommand{\fil}{\blacksquare}
\newcommand{\gap}{\square}
\newcommand{\sep}{\raisebox{0.9pt}{\ensuremath{\mspace{1mu}\wr\mspace{1mu}}}}
\newcommand{\filsep}{\raisebox{1pt}{\text{$\blacktriangleleft$}}}

% vectors
\makeatletter
\def\shortrightarrowfill@{\arrowfill@\relbar\relbar\shortrightarrow}
\newcommand{\ort}{\mathpalette{\overarrow@\shortrightarrowfill@}}
\makeatother
\makeatletter
\def\shortleftarrowfill@{\arrowfill@\relbar\relbar\shortleftarrow}
\newcommand{\olft}{\mathpalette{\overarrow@\shortleftarrowfill@}}
\makeatother
\makeatletter
\def\shortleftrightarrowfill@{\arrowfill@\relbar\relbar\leftrightarrow}
\newcommand{\olftrt}{\mathpalette{\overarrow@\shortleftrightarrowfill@}}
\makeatother
\newcommand{\til}[1]{\widetilde{#1}}

% formulas
\newcommand{\nin}{\not\in}
\newcommand{\sat}{\vDash}
\newcommand{\nsat}{\nvDash}
\newcommand{\et}{\;\wedge\;}
\newcommand{\vel}{\;\vee\;}
\newcommand{\then}{\;\rightarrow\;}
\newcommand{\Then}{\;\Rightarrow\;}
\renewcommand{\iff}{\;\leftrightarrow\;}
\newcommand{\Iff}{\;\Leftrightarrow\;}
\newcommand{\fa}[1]{\forall{\;#1}.\;}
\newcommand{\ex}[1]{\exists{\;#1}.\;}
\newcommand{\exinfinite}[1]{\exists^{\omega}{\;#1}.\;}
\newcommand{\exfinite}[1]{\exists^{<\omega}{\;#1}.\;}
\newcommand{\nex}[1]{\nexists{\;#1}.\;}

% sets, tuples, ...
\newcommand{\set}[1]{{\{ #1 \}}}
\newcommand{\bigset}[1]{{\bigl\{ #1 \bigr\}}}
\newcommand{\biggset}[1]{{\left\{ #1 \right\}}}
\newcommand{\settc}[2]{{\{ #1 \,:\, #2 \}}}
\newcommand{\bigsettc}[2]{{\bigl\{ #1 \,:\,#2 \bigr\}}}
\newcommand{\biggsettc}[2]{{\left\{ #1 \,:\,#2 \right\}}}
\newcommand{\ang}[1]{{\langle #1 \rangle}}
\newcommand{\bigang}[1]{{\bigl\langle #1 \bigr\rangle}}
\newcommand{\biggang}[1]{{\left\langle #1 \right\rangle}}
\newcommand{\intr}[1]{{\llbracket #1 \rrbracket}}
\newcommand{\bigintr}[1]{{\bigl\llbracket #1 \bigr\rrbracket}}
\newcommand{\biggintr}[1]{{\left\llbracket #1 \right\rrbracket}}
\newcommand{\len}[1]{{\lvert #1 \rvert}}
\newcommand{\biglen}[1]{{\bigl\lvert #1 \bigr\rvert}}
\newcommand{\bigglen}[1]{{\left\lvert #1 \right\rvert}}
\newcommand{\dlen}[1]{{\lVert #1 \rVert}}
\newcommand{\bigdlen}[1]{{\bigl\lVert #1 \bigr\rVert}}
\newcommand{\biggdlen}[1]{{\left\lVert #1 \right\rVert}}
\newcommand{\occ}[2]{\len{#2}_{#1}}
\newcommand{\bigocc}[2]{\biglen{#2}_{#1}}
\newcommand{\biggocc}[2]{\bigglen{#2}_{#1}}
\newcommand{\prj}[2]{\mspace{2mu}\downarrow_{#1}\mspace{-5mu}{#2}}

% relations
\newcommand{\trans}[2][]{\raisebox{-1pt}[10pt][0pt]{$\overset{#2}{\underset{^{#1}}{\raisebox{0pt}[3pt][0pt]{$\relbar\mspace{-8mu}\rightarrow$}}}$}}
\newcommand{\ftrans}[2][]{\raisebox{-1pt}[10pt][0pt]{$\overset{#2}{\underset{^{#1}}{\raisebox{0pt}[3pt][0pt]{$\relbar\mspace{-8mu}\circledcirc\mspace{-7.5mu}\rightarrow$}}}$}}
\newcommand{\noftrans}[2][]{\raisebox{-1pt}[10pt][0pt]{$\overset{#2}{\underset{^{#1}}{\raisebox{0pt}[3pt][0pt]{$\relbar\mspace{-8mu}\otimes\mspace{-7.5mu}\rightarrow$}}}$}}
\newcommand{\leads}[1]{\hookrightarrow^{#1}}
\newcommand{\leadsconst}[2]{\hookrightarrow^{#1}_{^{(#2)}}}
\newcommand{\groupsinto}{\trianglelefteq}
\newcommand{\finerthan}{\preceq}
\newcommand{\subgran}{\sqsubseteq}
\newcommand{\border}{\dashv}
\newcommand{\maxborder}{\dashv\!\!\dashv}
\newcommand{\notborder}{\not\dashv}
\newcommand{\notmaxborder}{\not\maxborder}
\newcommand{\dsim}{\approx}
\newcommand{\quotient}[1]{/\mspace{-4mu}#1}
\newcommand{\entails}{\rightvdash}

% operators
%\DeclareMathOperator{\lcm}{lcm}
\newcommand{\dom}{{\cD\mit{om}}}
\newcommand{\img}{{\cI\mspace{-2mu}\mit{mg}}}
\newcommand{\fr}{{\cF\mspace{-2mu}\mit{r}}}
\newcommand{\bch}{{\cB\mspace{-2mu}\mit{ch}}}
\newcommand{\infocc}{{\cI\mspace{-2mu}\mit{nf}}}
\newcommand{\unf}{\cU\mspace{-2mu}\mit{nf}}
\newcommand{\nop}{\mathtt{nop}}
\renewcommand{\b}[2]{\bigl(\begin{smallmatrix} #1 \\ #2 \end{smallmatrix}\bigr)}
\newcommand{\bb}[2]{\text{\small $\bigl(\begin{smallmatrix} #1 \\ #2 \end{smallmatrix}\bigr)$}}
\newcommand{\bbb}[2]{\text{\scriptsize $\bigl(\begin{smallmatrix} #1 \\ #2 \end{smallmatrix}\bigr)$}}
\renewcommand{\t}[3]{\biggl(\begin{smallmatrix} #1 \\ #2 \\ #3 \end{smallmatrix}\biggr)}
\renewcommand{\tt}[3]{\text{\small $\biggl(\begin{smallmatrix} #1 \\ #2 \\ #3 \end{smallmatrix}\biggr)$}}
\newcommand{\ttt}[3]{\text{\scriptsize $\biggl(\begin{smallmatrix} #1 \\ #2 \\ #3 \end{smallmatrix}\biggr)$}}

% complexity
\newcommand{\lowerbound}[1]{\Omega(#1)}
\newcommand{\biglowerbound}[1]{\Omega\bigl(#1\bigr)}
\newcommand{\bigglowerbound}[1]{\Omega\left(#1\right)}
\newcommand{\upperbound}[1]{\cO(#1)}
\newcommand{\bigupperbound}[1]{\cO\bigl(#1\bigr)}
\newcommand{\biggupperbound}[1]{\cO\left(#1\right)}
\newcommand{\comparable}[1]{\Theta(#1)}
\newcommand{\bigcomparable}[1]{\Theta\bigl(#1\bigr)}
\newcommand{\biggcomparable}[1]{\Theta\left(#1\right)}

